Causal Razors

When performing causal discovery, assumptions have to be made on how the true causal mechanism corresponds to the underlying joint probability distribution. These assumptions are labeled as causal razors in this work. We review numerous causal razors that appeared in the literature, and offer a comprehensive logical comparison of them. In particular, we scrutinize an unpopular causal razor, namely parameter minimality, in multinomial causal models and its logical relations with other well-studied causal razors. Our logical result poses a dilemma in selecting a reasonable scoring criterion for score-based casual search algorithms.

==> fig_diff_MEC.tex <==
\begin{center}
\subfloat{
\begin{tikzpicture}[scale=1.5, roundnode/.style={circle, draw=black!60, very thick, minimum size=5mm}]
\node (X1) at (0.0,1.0) {$1$};
\node (X2) at (0.9510565162951535,0.30901699437494745) {$2$};
\node (X3) at (0.5877852522924732,-0.8090169943749473) {$3$};
\node (X4) at (-0.587785252292473,-0.8090169943749476) {$4$};
\node (X5) at (-0.9510565162951536,0.30901699437494723) {$5$};
\node (label) at (0, -1.2) {(a) $\G^* = \G_{\pi^1} = \G_{\pi^2}$};
\path [->,line width=0.5mm] (X1) edge (X3);
\path [->,line width=0.5mm] (X2) edge (X3);
\path [->,line width=0.5mm] (X1) edge (X4);
\path [->,line width=0.5mm] (X3) edge (X5);
\path [->,line width=0.5mm] (X4) edge (X5);
\path [->,line width=0.5mm] (X1) edge (X5);
\end{tikzpicture}}
\hspace{1.5cm}
\subfloat{
\begin{tikzpicture}[scale=1.5, roundnode/.style={circle, draw=black!60, very thick, minimum size=5mm}]
\node (X1) at (0.0,1.0) {$1$};
\node (X2) at (0.9510565162951535,0.30901699437494745) {$2$};
\node (X3) at (0.5877852522924732,-0.8090169943749473) {$3$};
\node (X4) at (-0.587785252292473,-0.8090169943749476) {$4$};
\node (X5) at (-0.9510565162951536,0.30901699437494723) {$5$};
\node (label) at (0, -1.2) {(b) $\G_{\tau^1}$};
\path [->,line width=0.5mm] (X2) edge (X1);
\path [->,line width=0.5mm] (X2) edge (X3);
\path [->,line width=0.5mm] (X2) edge (X4);
\path [->,line width=0.5mm] (X2) edge (X5);
\path [->,line width=0.5mm] (X3) edge (X1);
\path [->,line width=0.5mm] (X3) edge (X4);
\path [->,line width=0.5mm] (X3) edge (X5);
\path [->,line width=0.5mm] (X4) edge (X1);
\path [->,line width=0.5mm] (X4) edge (X5);
\path [->,line width=0.5mm] (X5) edge (X1);
\end{tikzpicture}}
\hspace{1.5cm}
\subfloat{
\begin{tikzpicture}[scale=1.5, roundnode/.style={circle, draw=black!60, very thick, minimum size=5mm}]
\node (X1) at (0.0,1.0) {$1$};
\node (X2) at (0.9510565162951535,0.30901699437494745) {$2$};
\node (X3) at (0.5877852522924732,-0.8090169943749473) {$3$};
\node (X4) at (-0.587785252292473,-0.8090169943749476) {$4$};
\node (X5) at (-0.9510565162951536,0.30901699437494723) {$5$};
\node (label) at (0, -1.2) {(c) $\G_{\tau^2}$};
\path [->,line width=0.5mm] (X2) edge (X1);
\path [->,line width=0.5mm] (X2) edge (X3);
\path [->,line width=0.5mm] (X2) edge (X5);
\path [->,line width=0.5mm] (X3) edge (X1);
\path [->,line width=0.5mm] (X3) edge (X5);
\path [->,line width=0.5mm] (X4) edge (X1);
\path [->,line width=0.5mm] (X4) edge (X3);
\path [->,line width=0.5mm] (X4) edge (X5);
\path [->,line width=0.5mm] (X5) edge (X1);
\end{tikzpicture}}
\end{center}



==> ref.tex <==
@article{chickering2002optimal,
  title={Optimal structure identification with greedy search},
  author={Chickering, David Maxwell},
  journal={Journal of machine learning research},
  volume={3},
  pages={507--554},
  year={2002}
}

@book{spirtes2000causation,
  title={Causation, Prediction, and Search},
  author={Spirtes, Peter and Glymour, Clark and Scheines, Richard},
  year={2000},
  publisher={MIT press}
}

@article{raskutti2018learning,
  title={Learning directed acyclic graph models based on sparsest permutations},
  author={Raskutti, Garvesh and Uhler, Caroline},
  journal={Stat},
  volume={7},
  year={2018},
  publisher={Wiley Online Library}
}

@inproceedings{teyssier2005ordering,
  title={Ordering-based search: a simple and effective algorithm for learning {B}ayesian networks},
  author={Teyssier, Marc and Koller, Daphne},
  booktitle={Proceedings of the Conference on Uncertainty in Artificial Intelligence},
  pages={584--590},
  year={2005}
}

@inproceedings{verma1988causal,
  title={Causal networks: semantics and expressiveness},
  author={Verma, Thomas and Pearl, Judea},
  booktitle={Proceedings of the Conference on Uncertainty in Artificial Intelligence},
  pages={69--78},
  year={1988}
}

@article{solus2021consistency,
  author={Solus, Liam and Wang, Yuhao and Uhler, Caroline},
  title={Consistency guarantees for greedy permutation-based causal inference algorithms},
  journal={Biometrika},
  volume={108},
  pages={795-814},
  year={2021}
}

@inproceedings{lu2021improving,
  title={Improving causal discovery by optimal {B}ayesian network learning},
  author={Lu, Ni Y and Zhang, Kun and Yuan, Changhe},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  pages={8741--8748},
  year={2021}
}

@article{schwarz1978estimating,
  title={Estimating the dimension of a model},
  author={Schwarz, Gideon},
  journal={The annals of statistics},
  pages={461--464},
  year={1978},
  publisher={JSTOR}
}

@article{haughton1988choice,
  title={On the choice of a model to fit data from an exponential family},
  author={Haughton, Dominique MA},
  journal={The annals of statistics},
  pages={342--355},
  year={1988},
  publisher={JSTOR}
}

@article{margaritis1999bayesian,
  title={Bayesian network induction via local neighborhoods},
  author={Margaritis, Dimitris and Thrun, Sebastian},
  journal={Advances in neural information processing systems},
  volume={12},
  year={1999}
}

@inproceedings{friedman1999learning,
  title={Learning {B}ayesian network structure from massive datasets: the ``sparse candidate'' algorithm},
  author={Friedman, Nir and Nachman, Iftach and Pe{\'e}r, Dana},
  booktitle={Proceedings of the conference on Uncertainty in artificial intelligence},
  pages={206--215},
  year={1999}
}

@inproceedings{ramsey2006,
  title={Adjacency-faithfulness and conservative causal inference},
  author={Ramsey, Joseph and Zhang, Jiji and Spirtes, Peter},
  booktitle={Proceedings of the conference on Uncertainty in artificial intelligence},
  pages={401--408},
  year={2006}
}

@inproceedings{pearl1986graphoids,
  title={Graphoids: Graph-Based Logic for Reasoning about Relevance  Relations or When Would $x$ Tell You More about $y$ If You Already Know $z$?},
  author={Pearl, Judea and Paz, Azaria},
  booktitle={Proceedings of the European Conference on Artificial Intelligence},
  pages={357–363},
  year={1986}
}

@article{statnikov2013algorithms,
  title={Algorithms for discovery of multiple {M}arkov boundaries},
  author={Statnikov, Alexander and Lemeir, Jan and Aliferis, Constantin},
  journal={The Journal of Machine Learning Research},
  volume={14},
  pages={499--566},
  year={2013},
  publisher={JMLR}
}

@article{uhler2013geometry,
  title={Geometry of the faithfulness assumption in causal inference},
  author={Uhler, Caroline and Raskutti, Garvesh and B{\"u}hlmann, Peter and Yu, Bin},
  journal={The Annals of Statistics},
  pages={436--463},
  year={2013},
  publisher={JSTOR}
}

@article{zhang2013comparison,
  title={A comparison of three {O}ccam's razors for {M}arkovian causal models},
  author={Zhang, Jiji},
  journal={The British journal for the philosophy of science},
  volume={64},
  pages={423--448},
  year={2013},
  publisher={Oxford University Press}
}

@article{forster2020frugal,
  title={The frugal inference of causal relations},
  author={Forster, Malcolm and Raskutti, Garvesh and Stern, Reuben and Weinberger, Naftali},
  journal={The British Journal for the Philosophy of Science},
  year={2020},
  publisher={The University of Chicago Press}
}

@article{mohammadi2018generalized,
  title={Generalized permutohedra from probabilistic graphical models},
  author={Mohammadi, Fatemeh and Uhler, Caroline and Wang, Charles and Yu, Josephine},
  journal={SIAM Journal on Discrete Mathematics},
  volume={32},
  pages={64--93},
  year={2018},
  publisher={SIAM}
}

@inproceedings{Chickering1995,
author = {Chickering, David Maxwell},
title = {A Transformational Characterization of Equivalent {B}ayesian Network Structures},
year = {1995},
publisher = {Morgan Kaufmann Publishers Inc.},
address = {San Francisco, CA, USA},
booktitle = {Proceedings of the Conference on Uncertainty in Artificial Intelligence},
pages = {87–98},
numpages = {12},
}

@book{Pearl_10.5555/534975,
author = {Pearl, Judea},
title = {Probabilistic Reasoning in Intelligent Systems: Networks of Plausible Inference},
year = {1988},
publisher = {Morgan Kaufmann Publishers Inc.},
}

@book{Studeny_book,
  title={Probabilistic Conditional Independence Structures},
  author={Studen{\'y}, Milan},
  series={Information Science and Statistics},
  year={2005},
  publisher={Springer}
}

@inproceedings{vsimecek2006gaussian,
  title={{G}aussian representation of independence models over four random variables},
  author={{\v{S}}imecek, Petr},
  booktitle={Proccedings of the International Conference on Computational Statistics},
  year={2006},
  organization={Citeseer}
}

@inproceedings{vsimecek2006short,
  title={A short note on discrete representability of independence models},
  author={{\v{S}}imecek, Petr},
  booktitle={Proccedings of the Workshop on Probabilistic Graphical Models},
  pages={287--292},
  year={2006},
  organization={Citeseer}
}

@inproceedings{ogarrio2016hybrid,
  title={A hybrid causal search algorithm for latent variable models},
  author={Ogarrio, Juan Miguel and Spirtes, Peter and Ramsey, Joe},
  booktitle={Conference on probabilistic graphical models},
  pages={368--379},
  year={2016},
  organization={PMLR}
}

@misc{Dua:2019 ,
author = "Dua, Dheeru and Graff, Casey",
year = "2017",
title = "{UCI} Machine Learning Repository",
url = "http://archive.ics.uci.edu/ml",
institution = "University of California, Irvine, School of Information and Computer Sciences" }

@inproceedings{huang2018generalized,
  title={Generalized score functions for causal discovery},
  author={Huang, Biwei and Zhang, Kun and Lin, Yizhu and Sch{\"o}lkopf, Bernhard and Glymour, Clark},
  booktitle={Proceedings of the ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1551--1560},
  year={2018}
}

@article{10.1214/aos/1176350709,
author = {Dominique M. A. Haughton},
title = {On the Choice of a Model to Fit Data from an Exponential Family},
volume = {16},
journal = {The Annals of Statistics},
publisher = {Institute of Mathematical Statistics},
pages = {342 -- 355},
year = {1988}
}

@inproceedings{andrews2019learning,
  title={Learning high-dimensional directed acyclic graphs with mixed data-types},
  author={Andrews, Bryan and Ramsey, Joseph and Cooper, Gregory F},
  booktitle={The 2019 ACM SIGKDD Workshop on Causal Discovery},
  pages={4--21},
  year={2019},
  organization={PMLR}
}

@article{ZHANG20081873,
title = {On the completeness of orientation rules for causal discovery in the presence of latent confounders and selection bias},
journal = {Artificial Intelligence},
volume = {172},
pages = {1873-1896},
year = {2008},
author = {Jiji Zhang}
}

@article{raghu2018comparison,
  title={Comparison of strategies for scalable causal discovery of latent variable models from mixed data},
  author={Raghu, Vineet K and Ramsey, Joseph D and Morris, Alison and Manatakis, Dimitrios V and Sprites, Peter and Chrysanthis, Panos K and Glymour, Clark and Benos, Panayiotis V},
  journal={International journal of data science and analytics},
  volume={6},
  pages={33--45},
  year={2018},
  publisher={Springer}
}

@article{zheng2018dags,
  title={{DAG}s with no tears: Continuous optimization for structure learning},
  author={Zheng, Xun and Aragam, Bryon and Ravikumar, Pradeep K and Xing, Eric P},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}

@article{tsamardinos2006max,
  title={The max-min hill-climbing {B}ayesian network structure learning algorithm},
  author={Tsamardinos, Ioannis and Brown, Laura E and Aliferis, Constantin F},
  journal={Machine learning},
  volume={65},
  pages={31--78},
  year={2006},
  publisher={Springer}
}

@article{kalisch2012causal,
  title={Causal inference using graphical models with the {R} package pcalg},
  author={Kalisch, Markus and M{\"a}chler, Martin and Colombo, Diego and Maathuis, Marloes H and B{\"u}hlmann, Peter},
  journal={Journal of statistical software},
  volume={47},
  pages={1--26},
  year={2012}
}

@book{Kass:1437490,
      author        = "Kass, Robert E and Vos, Paul W",
      title         = "{Geometrical Foundations of Asymptotic Inference}",
      publisher     = "John Wiley \& Sons",
      address       = "Hoboken, NJ",
      year          = "2011"
}

@incollection{Spohn1994,
  author="Spohn, Wolfgang",
  editor="Humphreys, Paul",
  title="On the Properties of Conditional Independence",
  bookTitle="Patrick Suppes: Scientific Philosopher: Volume 1. Probability and Probabilistic Causality",
  year="1994",
  publisher="Springer Netherlands",
  pages="173--196"
}

@article{zhang2008detection,
  title={Detection of unfaithfulness and robust causal inference},
  author={Zhang, Jiji and Spirtes, Peter},
  journal={Minds and Machines},
  volume={18},
  number={2},
  pages={239--271},
  year={2008},
  publisher={Springer}
}

@book{Pearl2009Causality,
author = {Pearl, Judea},
title = {Causality: Models, Reasoning and Inference},
year = {2009},
publisher = {Cambridge University Press},
address = {USA},
edition = {2nd}
}

@inproceedings{ramsey2018tetrad,
  title={TETRAD—A toolbox for causal discovery},
  author={Ramsey, Joseph D and Zhang, Kun and Glymour, Madelyn and Romero, Ruben Sanchez and Huang, Biwei and Ebert-Uphoff, Imme and Samarasinghe, Savini and Barnes, Elizabeth A and Glymour, Clark},
  booktitle={8th International Workshop on Climate Informatics},
  year={2018}
}

@article{ramsey2017million,
  title={A million variables and more: the fast greedy equivalence search algorithm for learning high-dimensional graphical causal models, with an application to functional magnetic resonance images},
  author={Ramsey, Joseph and Glymour, Madelyn and Sanchez-Romero, Ruben and Glymour, Clark},
  journal={International journal of data science and analytics},
  volume={3},
  pages={121--129},
  year={2017},
  publisher={Springer}
}

@article{reisach2021beware,
  title={Beware of the Simulated DAG! Causal Discovery Benchmarks May Be Easy to Game},
  author={Reisach, Alexander and Seiler, Christof and Weichwald, Sebastian},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@article{shimizu2006linear,
  title={A linear non-Gaussian acyclic model for causal discovery.},
  author={Shimizu, Shohei and Hoyer, Patrik O and Hyv{\"a}rinen, Aapo and Kerminen, Antti and Jordan, Michael},
  journal={Journal of Machine Learning Research},
  volume={7},
  number={10},
  year={2006}
}

@inproceedings{GRaSP,
  title={Greedy relaxations of the sparsest permutation algorithm},
  author={Lam, Wai-Yin and Andrews, Bryan and Ramsey, Joseph},
  booktitle={Proceedings of the Thirty-Eighth Conference on Uncertainty in Artificial Intelligence},
  pages={1052--1062},
  year={2022},
  editor={Cussens, James and Zhang, Kun},
  volume={180},
  series ={Proceedings of Machine Learning Research},
  month={01--05 Aug},
  publisher={PMLR},
  pdf={https://proceedings.mlr.press/v180/lam22a/lam22a.pdf},
  url={https://proceedings.mlr.press/v180/lam22a.html}
}

@article{simecek_IM,
author = {Simecek, Petr},
year = {2007},
month = {01},
pages = {151-161},
title = {Independence models},
volume = {6},
journal = {Proceedings of 7th Workshop on Uncertainty processing WUPES}
}

@incollection{Geiger1990,
title = {On the logic of causal models},
editor = {Ross D. Shachter and Tod S. Levitt and Laveen N. Kanal and John F. Lemmer},
series = {Machine Intelligence and Pattern Recognition},
publisher = {North-Holland},
volume = {9},
pages = {3-14},
year = {1990},
booktitle = {Uncertainty in Artificial Intelligence},
issn = {0923-0459},
doi = {https://doi.org/10.1016/B978-0-444-88650-7.50006-8},
url = {https://www.sciencedirect.com/science/article/pii/B9780444886507500068},
author = {Dan Geiger and Judea Pearl}}

@article{ZhangSpirtes2011,
author = {Zhang, Jiji and Spirtes, Peter},
year = {2011},
month = {10},
pages = {335-347},
title = {Intervention, determinism, and the causal minimality condition},
volume = {182},
journal = {Synthese},
doi = {10.1007/s11229-010-9751-1}
}


@InProceedings{LinZhang2020,
  title = 	 {On learning causal structures from non-experimental data without any faithfulness assumption},
  author =       {Lin, Hanti and Zhang, Jiji},
  booktitle = 	 {Proceedings of the 31st International Conference  on Algorithmic Learning Theory},
  pages = 	 {554--582},
  year = 	 {2020},
  editor = 	 {Kontorovich, Aryeh and Neu, Gergely},
  volume = 	 {117},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {08 Feb--11 Feb},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v117/lin20a/lin20a.pdf},
  url = 	 {https://proceedings.mlr.press/v117/lin20a.html}
}

@misc{Zhalama2019asp,
      title={ASP-based Discovery of Semi-Markovian Causal Models under Weaker Assumptions}, 
      author={Zhalama and Jiji Zhang and Frederick Eberhardt and Wolfgang Mayer and Mark Junjie Li},
      year={2019},
      eprint={1906.02385},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{Ng_local_A_star,
 author = {Ng, Ignavier and Zheng, Yujia and Zhang, Jiji and Zhang, Kun},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {M. Ranzato and A. Beygelzimer and Y. Dauphin and P.S. Liang and J. Wortman Vaughan},
 pages = {20308--20320},
 publisher = {Curran Associates, Inc.},
 title = {Reliable Causal Discovery with Improved Exact Search and Weaker Assumptions},
 url = {https://proceedings.neurips.cc/paper/2021/file/a9b4ec2eb4ab7b1b9c3392bb5388119d-Paper.pdf},
 volume = {34},
 year = {2021}
}

@article{Weinberger_faithfulness,
title = "Faithfulness, Coordination, and Causal Coincidences",
author = "Naftali Weinberger",
year = "2017",
month = feb,
day = "15",
doi = "10.1007/s10670-017-9882-6",
language = "English",
journal = "Erkenntnis",
issn = "0165-0106",
publisher = "Springer",
}

@article{PC,
  title={An algorithm for fast recovery of sparse causal graphs},
  author={Spirtes, Peter and Glymour, Clark},
  journal={Social science computer review},
  volume={9},
  number={1},
  pages={62--72},
  year={1991},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@misc{Bryan_imset,
  doi = {10.48550/ARXIV.2207.08963},
  url = {https://arxiv.org/abs/2207.08963},
  author = {Andrews, Bryan and Cooper, Gregory F. and Richardson, Thomas S. and Spirtes, Peter},
  keywords = {Machine Learning (stat.ML), Machine Learning (cs.LG), Methodology (stat.ME), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {The m-connecting imset and factorization for ADMG models},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{Evans2014,
 ISSN = {00905364},
 URL = {http://www.jstor.org/stable/43556330},
 author = {Robin J. Evans and Thomas S. Richardson},
 journal = {The Annals of Statistics},
 number = {4},
 pages = {1452--1482},
 publisher = {Institute of Mathematical Statistics},
 title = {MARKOVIAN ACYCLIC DIRECTED MIXED GRAPHS FOR DISCRETE DATA},
 urldate = {2022-09-24},
 volume = {42},
 year = {2014}
}

@article{Hemmecke_imset,
title = {Characteristic imsets for learning Bayesian network structure},
journal = {International Journal of Approximate Reasoning},
volume = {53},
number = {9},
pages = {1336-1349},
year = {2012},
note = {Fifth European Workshop on Probabilistic Graphical Models (PGM-2010)},
issn = {0888-613X},
doi = {https://doi.org/10.1016/j.ijar.2012.04.001},
url = {https://www.sciencedirect.com/science/article/pii/S0888613X12000448},
author = {Raymond Hemmecke and Silvia Lindner and Milan Studený},
keywords = {Learning Bayesian network structure, Essential graph, Standard imset, Characteristic imset, LP relaxation of a polytope},
}

@article{Joe_GES_1M,
  author    = {Joseph D. Ramsey and
               Madelyn Glymour and
               Ruben Sanchez{-}Romero and
               Clark Glymour},
  title     = {A million variables and more: the Fast Greedy Equivalence Search algorithm
               for learning high-dimensional graphical causal models, with an application
               to functional magnetic resonance images},
  journal   = {Int. J. Data Sci. Anal.},
  volume    = {3},
  number    = {2},
  pages     = {121--129},
  year      = {2017},
  url       = {https://doi.org/10.1007/s41060-016-0032-z},
  doi       = {10.1007/s41060-016-0032-z},
  timestamp = {Fri, 11 Dec 2020 12:14:41 +0100},
  biburl    = {https://dblp.org/rec/journals/ijdsa/RamseyGSG17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Meek1995,
  title={Causal inference and causal explanation with background knowledge},
  author={Christopher Meek},
  booktitle={UAI},
  year={1995}
}

@article{Verma1990EquivalenceAS,
  title={Equivalence and Synthesis of Causal Models},
  author={Thomas Verma and Judea Pearl},
  journal={Probabilistic and Causal Inference},
  year={1990}
}

@article{kTriangle,
author = {Spirtes, Peter and Zhang, Jiji},
year = {2015},
month = {02},
pages = {},
title = {A Uniformly Consistent Estimator of Causal Effects under the $k$-Triangle-Faithfulness Assumption},
volume = {29},
journal = {Statistical Science},
doi = {10.1214/13-STS429}
}

@article{Andersen_CFC,
 ISSN = {00318248, 1539767X},
 URL = {http://www.jstor.org/stable/10.1086/673937}, 
 author = {Holly Andersen},
 journal = {Philosophy of Science},
 number = {5},
 pages = {672--683},
 publisher = {[The University of Chicago Press, Philosophy of Science Association]},
 title = {When to Expect Violations of Causal Faithfulness and Why It Matters},
 urldate = {2023-03-03},
 volume = {80},
 year = {2013}
}

@article{Children_node_simplicity,
author = {Bonawitz, Elizabeth and Lombrozo, Tania},
year = {2011},
month = {12},
pages = {1156-64},
title = {Occam's Rattle: Children's Use of Simplicity and Probability to Constrain Inference},
volume = {48},
journal = {Developmental psychology},
doi = {10.1037/a0026471}
}

@article{Richardson_MAGs,
 ISSN = {00905364},
 URL = {http://www.jstor.org/stable/1558693},
 abstract = {This paper introduces a class of graphical independence models that is closed under marginalization and conditioning but that contains all DAG independence models. This class of graphs, called maximal ancestral graphs, has two attractive features: there is at most one edge between each pair of vertices; every missing edge corresponds to an independence relation. These features lead to a simple parameterization of the corresponding set of distributions in the Gaussian case.},
 author = {Thomas Richardson and Peter Spirtes},
 journal = {The Annals of Statistics},
 number = {4},
 pages = {962--1030},
 publisher = {Institute of Mathematical Statistics},
 title = {Ancestral Graph Markov Models},
 urldate = {2023-04-01},
 volume = {30},
 year = {2002}
}

@phdthesis{MyPhD,
  author       = {Lam, Wai-Yin}, 
  title        = {Causal Razors and Causal Search Algorithms},
  school       = {Carnegie Mellon University},
  year         = 2023,
}

@article{Kalisch_strong_CFC,
  author  = {Markus Kalisch and Peter B{{\"u}}hlmann},
  title   = {Estimating high-dimensional directed acyclic graphs with the PC-algorithm},
  journal = {Journal of Machine Learning Research},
  year    = {2007},
  volume  = {8},
  number  = {22},
  pages   = {613--636},
  url     = {http://jmlr.org/papers/v8/kalisch07a.html}
}

@article{MacKay_1992,
    author = {MacKay, David J. C.},
    title = "{Bayesian interpolation}",
    journal = {Neural Computation},
    volume = {4},
    number = {3},
    pages = {415-447},
    year = {1992},
    month = {05},
    issn = {0899-7667},
    doi = {10.1162/neco.1992.4.3.415},
    url = {https://doi.org/10.1162/neco.1992.4.3.415},
    eprint = {https://direct.mit.edu/neco/article-pdf/4/3/415/812340/neco.1992.4.3.415.pdf},
}

@book{woodward2021causation,
  title={Causation with a Human Face: Normative Theory and Descriptive Psychology},
  author={Woodward, James},
  year={2021},
  publisher={Oxford University Press}
}

@article{lauritzenlectures,
  title={Lectures on graphical models},
  author={Lauritzen, Steffen L},
  url={http://web.math.ku.dk/~lauritzen/papers/gmnotes.pdf},
  year = {2019}
}

@book{Reichenbach,
	year = {1956},
	author = {Hans Reichenbach},
	publisher = {Mineola, N.Y.: Dover Publications},
	title = {The Direction of Time}
}

@article{Strobl_nonparametric_CI_test,
url = {https://doi.org/10.1515/jci-2018-0017},
title = {Approximate kernel-based conditional independence tests for fast non-parametric causal discovery},
author = {Eric V. Strobl and Kun Zhang and Shyam Visweswaran},
pages = {20180017},
volume = {7},
number = {1},
journal = {Journal of Causal Inference},
doi = {doi:10.1515/jci-2018-0017},
year = {2019}}

@article{Abductive_node_simplicity,
author = {Lombrozo, Tania},
year = {2012},
month = {01},
pages = {260-276},
title = {Explanation and abductive inference},
journal = {Oxford Handbook of Thinking and Reasoning},
doi = {10.1093/oxfordhb/9780199734689.013.0014}
}

@article{Bayesian_Razor_of_People,
author = {Blanchard, Thomas and Lombrozo, Tania and Nichols, Shaun},
title = {Bayesian Occam's razor is a razor of the people},
journal = {Cognitive Science},
volume = {42},
number = {4},
pages = {1345-1359},
doi = {https://doi.org/10.1111/cogs.12573},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/cogs.12573},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/cogs.12573},
year = {2018}
}

@article{pacer_ockham,
  title={Ockham’s razor cuts to the root: Simplicity in causal explanation},
  author={Pacer, M and Lombrozo, Tania},
  journal={Journal of Experimental Psychology: General},
  volume={146},
  number={12},
  pages={1761},
  year={2017},
  publisher={American Psychological Association}
}
